Deep Agent: Studying the Dynamics of Information Spread and Evolution in Social Networks

This paper explains the design of a social network analysis framework, developed under DARPA's SocialSim program, with novel architecture that models human emotional, cognitive and social factors. Our framework is both theory and data-driven, and utilizes domain expertise. Our simulation effort helps in understanding how information flows and evolves in social media platforms. We focused on modeling three information domains: cryptocurrencies, cyber threats, and software vulnerabilities for the three interrelated social environments: GitHub, Reddit, and Twitter. We participated in the SocialSim DARPA Challenge in December 2018, in which our models were subjected to extensive performance evaluation for accuracy, generalizability, explainability, and experimental power. This paper reports the main concepts and models, utilized in our social media modeling effort in developing a multi-resolution simulation at the user, community, population, and content levels.

==> glossary.tex <==
%%%%%%%%%%%%%%%%%%%%%%acronym.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample list of acronyms
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\Extrachap{Glossary}


Use the template \emph{glossary.tex} together with the Springer document class SVMono (monograph-type books) or SVMult (edited books) to style your glossary\index{glossary} in the Springer layout.


\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

==> part.tex <==
%%%%%%%%%%%%%%%%%%%%%part.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% sample part title
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{partbacktext}
\part{Part Title}
\noindent Use the template \emph{part.tex} together with the Springer document class SVMono (monograph-type books) or SVMult (edited books) to style your part title page and, if desired, a short introductory text (maximum one page) on its verso page in the Springer layout.

\end{partbacktext}

==> untitled folder/glossary.tex <==
%%%%%%%%%%%%%%%%%%%%%%acronym.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample list of acronyms
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\Extrachap{Glossary}


Use the template \emph{glossary.tex} together with the Springer document class SVMono (monograph-type books) or SVMult (edited books) to style your glossary\index{glossary} in the Springer layout.


\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

\runinhead{glossary term} Write here the description of the glossary term. Write here the description of the glossary term. Write here the description of the glossary term.

==> untitled folder/part.tex <==
%%%%%%%%%%%%%%%%%%%%%part.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% sample part title
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{partbacktext}
\part{Part Title}
\noindent Use the template \emph{part.tex} together with the Springer document class SVMono (monograph-type books) or SVMult (edited books) to style your part title page and, if desired, a short introductory text (maximum one page) on its verso page in the Springer layout.

\end{partbacktext}

==> untitled folder/referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%


\begin{thebibliography}{99.}%

\bibitem{adamic2016information}
Lada~A Adamic, Thomas~M Lento, Eytan Adar, and Pauline~C Ng.
\newblock Information evolution in social networks.
\newblock In {\em Proceedings of the Ninth ACM International Conference on Web
  Search and Data Mining}, pages 473--482. ACM, 2016.

% \bibitem{barabasi1999mean}
% Albert-L{\'a}szl{\'o} Barab{\'a}si, R{\'e}ka Albert, and Hawoong Jeong.
% \newblock Mean-field theory for scale-free random networks.
% \newblock {\em Physica A: Statistical Mechanics and its Applications},
%   272(1-2):173--187, 1999.

\bibitem{bass1969new}
Frank~M Bass.
\newblock A new product growth for model consumer durables.
\newblock {\em Management science}, 15(5):215--227, 1969.

\bibitem{bass2004new}
Frank~M Bass.
\newblock A new product growth for model consumer durables.
\newblock {\em Management science}, 50(12\_supplement):1825--1832, 2004.

\bibitem{centola2007complex}
Damon Centola and Michael Macy.
\newblock Complex contagions and the weakness of long ties.
\newblock {\em American journal of Sociology}, 113(3):702--734, 2007.

% \bibitem{dodds2004universal}
% Peter~Sheridan Dodds and Duncan~J Watts.
% \newblock Universal behavior in a generalized model of contagion.
% \newblock {\em Physical review letters}, 92(21):218701, 2004.

\bibitem{epstein2014agent_zero}
Joshua~M Epstein.
\newblock {\em Agent\_zero: Toward neurocognitive foundations for generative
  social science}, volume~25.
\newblock Princeton University Press, 2014.

% \bibitem{garibay2019agent}
% Ivan Garibay, Chathika Gunaratne, Niloofar Yousefi, and Steve Scheinert.
% \newblock The agent-based model canvas: A modeling lingua franca for
%   computational social science.
% \newblock {\em Social-Behavioral Modeling for Complex Systems}, pages 521--544,
%   2019.

\bibitem{gintis2015homo}
Herbert Gintis, Dirk Helbing, et~al.
\newblock Homo socialis: An analytical core for sociological theory.
\newblock {\em Review of Behavioral Economics}, 2(1-2):1--59, 2015.

\bibitem{goldenberg2001talk}
Jacob Goldenberg, Barak Libai, and Eitan Muller.
\newblock Talk of the network: A complex systems look at the underlying process
  of word-of-mouth.
\newblock {\em Marketing letters}, 12(3):211--223, 2001.

\bibitem{goldenberg2001using}
Jacob Goldenberg, Barak Libai, and Eitan Muller.
\newblock Using complex systems analysis to advance marketing theory
  development: Modeling heterogeneity effects on new product growth through
  stochastic cellular automata.
\newblock {\em Academy of Marketing Science Review}, 9(3):1--18, 2001.

\bibitem{granovetter1978threshold}
Mark Granovetter.
\newblock Threshold models of collective behavior.
\newblock {\em American journal of sociology}, 83(6):1420--1443, 1978.

\bibitem{gunaratne2017alternate}
Chathika Gunaratne and Ivan Garibay.
\newblock Alternate social theory discovery using genetic programming: towards
  better understanding the artificial anasazi.
\newblock In {\em Proceedings of the Genetic and Evolutionary Computation
  Conference}, pages 115--122. ACM, 2017.

\bibitem{gunaratne2019multi}
Chathika Gunaratne, Chathurani Senevirathna, Chathura Jayalath, Nisha Baral,
  William Rand, and Ivan Garibay.
\newblock A multi-action cascade model of conversation.
\newblock In {\em 5th International Conference on Computational Social Science,
  URL http://app. ic2s2. org/app/sessions/9kXqn5btgKKC5yfCvg/details}, 2019.

\bibitem{NedaSHD}
Neda Hajiakhoond~Bidoki, Madeline Schiappa, Gita Sukthankar, and Ivan Garibay.
\newblock Predicting social network evolution from community data partitions.
\newblock {\em 2019 International Conference on Social Computing,
  Behavioral-Cultural Modeling and Prediction and Behavior Representation in
  Modeling and Simulation}, pages In--press, 2019.

% \bibitem{nguyen2013influence}
% Dung~T Nguyen, Soham Das, and My~T Thai.
% \newblock Influence maximization in multiple online social networks.
% \newblock In {\em 2013 IEEE Global Communications Conference (GLOBECOM)}, pages
%   3060--3065. IEEE, 2013.

\bibitem{rand2015agent}
William Rand, Jeffrey Herrmann, Brandon Schein, and Ne{\v{z}}a Vodopivec.
\newblock An agent-based model of urgent diffusion in social media.
\newblock {\em Journal of Artificial Societies and Social Simulation}, 18(2):1,
  2015.

\bibitem{rand2011agent}
William Rand and Roland~T Rust.
\newblock Agent-based modeling in marketing: Guidelines for rigor.
\newblock {\em International Journal of Research in Marketing}, 28(3):181--193,
  2011.

% \bibitem{scheinert2015shape}
% Steve Scheinert, Christopher Koliba, Stephanie Hurley, Sarah Coleman, and Asim
%   Zia.
% \newblock The shape of watershed governance: Locating the boundaries of
%   multiplex networks.
% \newblock {\em Complexity, Governance \& Networks}, 2(1):65--82, 2015.

\bibitem{vsuvakov2012agent}
Milovan {\v{S}}uvakov, David Garcia, Frank Schweitzer, and Bosiljka Tadi{\'c}.
\newblock Agent-based simulations of emotion spreading in online social
  networks.
\newblock {\em arXiv preprint arXiv:1205.6278}, 2012.

\bibitem{watts2002simple}
Duncan~J Watts.
\newblock A simple model of global cascades on random networks.
\newblock {\em Proceedings of the National Academy of Sciences},
  99(9):5766--5771, 2002.

% \bibitem{zhao2011herd}
% Li~Zhao, Guang Yang, Wei Wang, Yu~Chen, JP~Huang, Hirotada Ohashi, and H~Eugene
%   Stanley.
% \newblock Herd behavior in a complex adaptive system.
% \newblock {\em Proceedings of the National Academy of Sciences},
%   108(37):15058--15063, 2011.

\bibitem{basu2015multiplex}
Prithwish Basu, Matthew Dippel, and Ravi Sundaram.
\newblock Multiplex networks: A generative model and algorithmic complexity.
\newblock In {\em 2015 IEEE/ACM International Conference on Advances in Social
  Networks Analysis and Mining (ASONAM)}, pages 456--463. IEEE, 2015.

\bibitem{gunaratne2019theory}
Chathika Gunaratne, Nisha Baral, William Rand, Ivan Garibay, Chathura Jayalath,
  and Chathurani Senevirathna.
\newblock The effects of information overload on online conversation dynamics.
\newblock {\em Computational and Mathematical Organization Theory}, 2020.

\bibitem{mcpherson2001birds}
Miller McPherson, Lynn Smith-Lovin, and James~M Cook.
\newblock Birds of a feather: Homophily in social networks.
\newblock {\em Annual review of sociology}, 27(1):415--444, 2001.

\bibitem{saadat2018initializing}
Samaneh Saadat, Chathika Gunaratne, Nisha Baral, Gita Sukthankar, and Ivan
  Garibay.
\newblock Initializing agent-based models with clustering archetypes.
\newblock In {\em International Conference on Social Computing,
  Behavioral-Cultural Modeling and Prediction and Behavior Representation in
  Modeling and Simulation}, pages 233--239. Springer, 2018.





\end{thebibliography}

